LSNR: Learned Sparse News Recommendations with Attentive User Modeling

Current learned sparse approaches for recommender systems, such as STAR, represent a user by concatenating their interaction history into a single query string. For news, this creates two bottlenecks: concatenation collapses a user's distinct reading interests into one flat query, and, because news articles are long-form text, concatenating several news articles quickly overruns the context window of the language model used as backbone and forces quality-degrading truncation. To address both bottlenecks, we introduce learned sparse news recommendations (LSNR). LSNR encodes each article independently and constructs a sparse user vector by combining learned, attention-based weighting of the per-article sparse representations with a dense-projected expansion at the user level. Experiments on the MIND and EBNeRD datasets show that LSNR significantly outperforms STAR, with these gains holding even in short-history settings where truncation is not a factor. Compared to state-of-the-art dense recommenders, LSNR is competitive in standard settings and it outperforms them when the user history is short. An ablation of the user encoder confirms that learned attention-based aggregation outperforms simpler pooling alternatives. Beyond effectiveness, an additional advantage of LSNR is that it serves from an index an order of magnitude smaller than an uncompressed dense baseline.

==> tables/table-main-results.tex <==
\begin{table}[t!]
\caption{Performance of LSNR compared to BM25 and learned sparse baseline STAR across the full MIND and EBNeRD benchmarks. \textbf{Bold} denotes the highest score, $^\ast$ denotes a significant improvement over the second-best method ($p < 0.01$).}
\label{tab:sparse_results_full}
\small
\setlength{\tabcolsep}{3.2pt}
\centering
\begin{tabular}{l ccc ccc}
\toprule
 & \multicolumn{3}{c}{\bf MIND} & \multicolumn{3}{c}{\bf EBNeRD} \\
\cmidrule(lr){2-4} \cmidrule(lr){5-7}
\textbf{Method} & N@10 & N@5 & MRR & N@10 & N@5 & MRR \\
\midrule
BM25 & 0.3142 & 0.2541 & 0.2480 & 0.4639 & 0.3868 & 0.3503 \\
STAR & 0.3815 & 0.3191 & 0.2973 & 0.4704 & 0.3925 & 0.3459 \\
\midrule
\textbf{LSNR (Ours)} & \textbf{0.4234}\rlap{$^\ast$} & \textbf{0.3620}\rlap{$^\ast$} & \textbf{0.3310}\rlap{$^\ast$} & \textbf{0.5200}\rlap{$^\ast$} & \textbf{0.4547}\rlap{$^\ast$} & \textbf{0.4027}\rlap{$^\ast$} \\
\bottomrule
\end{tabular}
\end{table}

\begin{table}[t]
\caption{Short-history ($N=1$) performance of LSNR compared to BM25 and learned sparse baseline STAR. \textbf{Bold} denotes the highest score, $^\ast$ denotes a significant improvement over the second-best method ($p < 0.01$).}
\label{tab:short_history_sparse}
\small
\setlength{\tabcolsep}{3.2pt}
\centering
\begin{tabular}{l ccc ccc}
\toprule
 & \multicolumn{3}{c}{\bf MIND ($N=1$)} & \multicolumn{3}{c}{\bf EBNeRD ($N=1$)} \\
\cmidrule(lr){2-4} \cmidrule(lr){5-7}
\textbf{Method} & N@10 & N@5 & MRR & N@10 & N@5 & MRR \\
\midrule
BM25 & 0.3109 & 0.2505 & 0.2445 & 0.4359 & 0.3519 & 0.3203 \\
STAR & 0.3500 & 0.2880 & 0.2742 & 0.4656 & 0.3866 & 0.3408 \\
\midrule
\textbf{LSNR (Ours)} & \textbf{0.3626}\rlap{$^\ast$} & \textbf{0.3015}\rlap{$^\ast$} & \textbf{0.2819}\rlap{$^\ast$} & \textbf{0.5022}\rlap{$^\ast$} & \textbf{0.4317}\rlap{$^\ast$} & \textbf{0.3824}\rlap{$^\ast$} \\
\bottomrule
\end{tabular}
\end{table}

\begin{table*}[t!]
\caption{Comparison of LSNR against state-of-the-art dense news recommenders. \textbf{Bold} denotes the highest score, $^\ast$ denotes a significant improvement over the second-best method ($p < 0.01$).}
\label{tab:dense_comparison}
\centering
\begin{tabular}{l ccc ccc ccc ccc}
\toprule
 & \multicolumn{6}{c}{\bf Full-history users} & \multicolumn{6}{c}{\bf Short-history users ($N=1$)} \\
\cmidrule(lr){2-7} \cmidrule(lr){8-13}
 & \multicolumn{3}{c}{\bf MIND} & \multicolumn{3}{c}{\bf EBNeRD} & \multicolumn{3}{c}{\bf MIND} & \multicolumn{3}{c}{\bf EBNeRD} \\
\cmidrule(lr){2-4} \cmidrule(lr){5-7} \cmidrule(lr){8-10} \cmidrule(lr){11-13}
\textbf{Method} & N@10 & N@5 & MRR & N@10 & N@5 & MRR & N@10 & N@5 & MRR & N@10 & N@5 & MRR \\
\midrule
NRMS  & \textbf{0.4256} & \textbf{0.3641} & \textbf{0.3322} & 0.5290 & 0.4629 & 0.4119 & 0.3536 & 0.2927 & 0.2748 & 0.4880 & 0.4127 & 0.3679 \\
NAML  & 0.4247 & 0.3633 & 0.3320 & \textbf{0.5312} & \textbf{0.4649} & \textbf{0.4134} & 0.3301 & 0.2908 & 0.2723 & 0.4889 & 0.4134 & 0.3690 \\
LSTUR & 0.3794 & 0.3183 & 0.2943 & 0.5114 & 0.4407 & 0.3909 & 0.2806 & 0.2205 & 0.2168 & 0.4496 & 0.3655 & 0.3305 \\
\midrule
\textbf{LSNR} & 0.4234 & 0.3620 & 0.3310 & 0.5200 & 0.4547 & 0.4027 & \textbf{0.3626}\rlap{$^\ast$} & \textbf{0.3015}\rlap{$^\ast$} & \textbf{0.2819}\rlap{$^\ast$} & \textbf{0.5022}\rlap{$^\ast$} & \textbf{0.4317}\rlap{$^\ast$} & \textbf{0.3824}\rlap{$^\ast$} \\
\bottomrule
\end{tabular}
\end{table*}

